Eternal Vertex Cover on Bipartite and Co-Bipartite Graphs

Eternal Vertex Cover problem is a dynamic variant of the vertex cover problem. We have a two player game in which guards are placed on some vertices of a graph. In every move, one player (the attacker) attacks an edge. In response to the attack, the second player (defender) moves the guards along the edges of the graph in such a manner that at least one guard moves along the attacked edge. If such a movement is not possible, then the attacker wins. If the defender can defend the graph against an infinite sequence of attacks, then the defender wins. The minimum number of guards with which the defender has a winning strategy is called the Eternal Vertex Cover Number of the graph G. On general graphs, the computational problem of determining the minimum eternal vertex cover number is NP-hard and admits a 2-approximation algorithm and an exponential kernel. The complexity of the problem on bipartite graphs is open, as is the question of whether the problem admits a polynomial kernel. We settle both these questions by showing that Eternal Vertex Cover is NP-hard and does not admit a polynomial compression even on bipartite graphs of diameter six. We also show that the problem admits a polynomial time algorithm on the class of cobipartite graphs.

==> oldproof-dominatingset.tex <==

\begin{theorem}
The \EVC{} problem is \NPH{} even when restricted to the class of bipartite graphs.
\end{theorem}


\begin{proof}

We establish this by a reduction from \DS.  Let $\langle G = (V,E),k \rangle$ be an instance of \DS{}. We denote the vertices in $V$ by $\{x_1, \ldots, x_n\}$, and use $m$ to denote $|E|$. We assume that $G$ is connected, since \DS{} is \NPH{} even for connected graphs. Further, we assume that $k < n-2$ by returning a trivial \textsc{Yes}-instance of \EVC{} if $k \geq n-2$. The correctness of this follows from the fact that $(G,k)$ is already a \textsc{Yes} instance when $G$ is connected and $k \geq n-2$: the set of all vertices except for two leaves from a spanning tree of $G$ would serve as a valid dominating set for $G$.

\nmtodo{Add a definition of Dominating Set and a reference to it's NP-completeness in the prelims.}

\paragraph*{The Construction.} We will develop an instance of \EVC{} which we denote by $\langle H, \ell \rangle$ based on $\langle G,k \rangle$ as follows.

First, we introduce $n$ \emph{original} vertices, denoted by $A := \{v_i~|~1 \leq i \leq n\}$ and $n$ \emph{partner} vertices, denoted by $B := \{u_i~|~1 \leq i \leq n\}$. Next, for all $i \in [n]$, we add $n^2$ \emph{dependent} vertices of type $i$, denoted by $C_i := \{w^i_j~|~1\leq j \leq n^2\}$. Finally, we add two special vertices denoted by $\star$ and $\dagger$, which we will refer to as the \emph{universal} and \emph{backup} vertices respectively. To summarize, the vertex set consists of the following $2n + n^3 + 2$ vertices:

$$ V(H) := A \cup B \cup C_1 \cup \cdots \cup C_n \cup \{\star,\dagger\}.$$

We now describe the edges in $H$:

\begin{itemize}
\item There are $n$ \emph{matching} edges that connect every original vertex with a corresponding partner vertex, i.e, for all $i \in [n]$ we have the edge $(v_i,u_i)$.

\item There are $m$ \emph{structural} edges given by $(v_p,u_q)$ for every pair $(p,q)$ such that $(x_p,x_q) \in E(G)$. In other words, for every edge $(x_p,x_q)$ in the graph $G$, the original vertex $v_p$ is adjacent to the partner vertex $u_q$. Note that in the graph $H$ constructed so far, the degree of the vertex $u_i$ is one more than the degree of $x_i$ in $G$. 

\item The dependent vertices of type $i$ are adjacent to the $i^{th}$ partner vertex, i.e, for every $i \in [n]$, we have a \emph{sliding} edge $(u_i,w)$ for each $w \in C_i$. 

\item The universal vertex $\star$ is adjacent to every original vertex via a \emph{supplier} edge. In particular, for every $i \in [n]$, we have the edge $(v_i,\star)$. 

\item Finally, we have the edge $(\star,\dagger)$, indicating that the backup vertex $\dagger$ is adjacent to the universal vertex. We call this edge a \emph{bridge}. 

\end{itemize}

To summarize, we have the following edges in $H$:

\begin{equation} \label{eq1}
  \begin{split}
  E(H) & = \{(u_i,v_i)~|~ 1 \leq i \leq n\}~\longleftarrow \mbox{ the matching edges} \\
  & \cup \{(v_p,u_q)~|~ 1 \leq i,j \leq n \mbox{ and } (x_p,x_q) \in E(H)\}~\longleftarrow \mbox{ the structural edges}\\
  & \cup \{(u_1,w)~|~ w \in C_i)\} \longleftarrow \mbox{ the type } 1 \mbox{ sliding edges}\\
  & \cup \vdots \\
  & \cup \{(u_i,w)~|~ w \in C_i)\} \longleftarrow \mbox{ the type } i \mbox{ sliding edges}\\
  & \cup \vdots \\
  & \cup \{(u_n,w)~|~ w \in C_i)\}~\longleftarrow \mbox{ the type } n \mbox{ sliding edges}\\ 
  & \cup \{(v_i,\star)~|~ 1 \leq i \leq n\} ~\longleftarrow \mbox{ the supplier edges} \\
  & \cup \{(\star,\dagger)\}~\longleftarrow \mbox{the bridge edge}.
  \end{split}
  \end{equation}

We now let $\ell := n+k+2$, and this completes the description of the reduced instance $\langle H, \ell \rangle$. 

% \[ \cup_{1 \leq i \leq n} \{u_i, v_i\} \cup \cup_{1 \leq i \leq n} \{w_j^{i} ~|~ 1 \leq j \leq n^2 \} \cup \{\star,\dagger\} \] 

% \begin{itemize}
% \item $n$ \emph{original} vertices, denoted by $A := \{v_i~|~1 \leq i \leq n\}$ and $n$ \emph{partner} vertices, denoted by $B := \{u_i~|~1 \leq i \leq n\}$, 
% \item for each $1 \leq i \leq n$, $n^2$ \emph{guard} vertices of type $i$, denoted by $C_i := \{w^i_j~|~1 \leq j \leq n^2\}$, 
% \end{itemize}

\begin{claim}
  The vertex cover number of $H$ is $n+1$. 
\end{claim}

\begin{proof}
  This follows from the fact that the $n$ matching edges in $H$ form a matching (showing the lower bound), and that $B \cup \{\star\}$ is a vertex cover in $H$ (which implies the upper bound).
\end{proof}

\begin{claim}
  \label{claim-invariant}
  Any vertex cover of $H$ that has at most $\ell$ vertices must contain $B \cup \{\star\}$. 
\end{claim}

\begin{proof}
  Consider a vertex cover $S \subseteq V(H)$ that does not contain some partner vertex $v_i \in B$. Then $S$ must contain all the $n^2$ dependent vertices in $C_i$, but since $|C_i| = n^2$, this contradicts our assumption that $|S| \leq \ell$. 

  Now consider again a vertex cover $S \subseteq V(H)$ that does not contain $\star$. Observe that we already know that $B \subseteq S$. If $S$ does not contain $\star$, then $A \subseteq S$, and this implies that $|S| \geq |A| + |B| = 2n$; however, $\ell = n + k + 2 < 2n$ (recall that $k < n - 2$), and this is a contradiction. 
\end{proof}


\paragraph*{The Forward Direction.} Suppose $\langle G = (V,E),k \rangle$ is a \textsc{Yes}-instance of \DS. We argue that $\langle H, \ell \rangle$ is a \textsc{Yes}-instance of \EVC{}.

Let $S \subseteq V(G)$ be a dominating set of $G$. Without loss of generality (by renaming), we assume that $S = \{x_1, \ldots, x_k\}$. Let $S^\star := \{v_1, \ldots, v_k\} \subseteq A$, i.e, the original vertices of $H$ corresponding to the solution in $G$. 

Note that all the following are vertex covers of size $n + k + 2$ for $H$:

\begin{itemize}
\item A backup vertex cover is given by $X := B \cup \{\star\} \cup S^\star \cup \{\dagger\}$.
\item A dependent vertex cover of type $i$ is given by $Y_i := B \cup \{\star\} \cup S^\star \cup \{w\}$, where $w$ is a dependent vertex from $C_i$.
\item A original vertex cover given by $Z_j := B \cup \{\star\} \cup S^\star \cup \{v_j\}$, for some $j > k$.
\end{itemize}

We remark that there may other vertex covers of size $n + k + 2$ that don't ``fit'' into any of the categories listed above. A vertex cover that is either a backup, dependent, or original vertex cover is called a \emph{nice} vertex cover.

We argue that if guards are occupying a nice vertex cover, then any attack can be defended by moving guards along edges in such a way that the new configuration also corresponds to a nice vertex cover. This implies that any sequence of attacks can be defended, by starting with an arbitrary nice vertex cover.

% \begin{claim}
  % Let $\mathcal{S} \subseteq V(H)$ be a nice vertex cover, and let $e \in E(H)$. If the guards are currently occupying $\mathcal{S}$, it is possible to move every guard at most once to a neighboring vertex so that the attack on $e$ is defended, and the new positions of the guards also corresponds to a nice vertex cover. 
% \end{claim}

\begin{claim}
  Let $\mathcal{S} \subseteq V(H)$ be a nice vertex cover, and let $e \in E(H)$. If the guards are currently occupying $\mathcal{S}$, there is a legal move that defends $e$ such that the new position of the guards also corresponds to a nice vertex cover. 
\end{claim}

\begin{proof}

  We argue this by an exhaustive case analysis on $(\mathcal{S},e)$.

  \paragraph*{Case 1. $\mathcal{S}$ is a backup vertex cover and $e$ is a matching edge.}

  Let $e = (u_i,v_i)$. If $i \leq k$, the guards on $u_i$ and $v_i$ exchange positions. If $i > k$, let $q \in [k]$ be such that $(x_q,x_i) \in E(G)$. We now perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $v_i$ along the matching edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; and 
    \item the guard on $\dagger$ moves to $\star$ along the bridge.
  \end{itemize}

  Note that this new configuration of guards corresponds to a original vertex cover. 

  \paragraph*{Case 2. $\mathcal{S}$ is a backup vertex cover and $e$ is a structural edge.}

  Let $e = (v_q,u_p)$. If $q \leq k$, then the guards on $v_q$ and $u_p$ exchange positions. Otherwise, suppose $p \leq k$. Then, we perform the following sequence of moves:

  \begin{itemize}
    \item The guard on $u_p$ moves to $v_q$ along the structural edge that was attacked;
    \item the guard on $v_p$ moves to $u_p$ along a matching edge; 
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; and 
    \item the guard on $\dagger$ moves to $\star$ along the bridge.
  \end{itemize}

  However, if $p > k$, then let $r \in [k]$ be such that $(x_r,x_p) \in E(G)$. We now perform the following sequence of moves:

  \begin{itemize}
    \item The guard on $u_p$ moves to $v_q$ along the structural edge that was attacked;
    \item the guard on $v_r$ moves to $u_p$ along a structural edge;
    \item the guard on the universal vertex moves to $v_r$ along a supplier edge; and 
    \item the guard on $\dagger$ moves to $\star$ along the bridge.
  \end{itemize}

  \paragraph*{Case 3. $\mathcal{S}$ is a backup vertex cover and $e$ is a sliding edge.}

  Let $i \in [n]$ and suppose $e = (u_i,w)$ for some $w \in C_i$. Suppose $i \leq k$. Then we have the following sequence of moves. 

  \begin{itemize}
    \item the guard on $u_i$ moves to $w$ along the sliding edge that was attacked;
    \item the guard on $v_i$ moves to $u_i$ along a matching edge;
    \item the guard on the universal vertex moves to $v_i$ along a supplier edge; and 
    \item the guard on $\dagger$ moves to $\star$ along the bridge.
  \end{itemize}

  Now suppose $i > k$ and let $q \in [k]$ be such that $(x_q,x_i) \in E(G)$. We now perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $w$ along the sliding edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; and 
    \item the guard on $\dagger$ moves to $\star$ along the bridge.
  \end{itemize}

  In both cases, the new configuration of the guards corresponds to a dependent vertex cover. 

  \paragraph*{Case 4. $\mathcal{S}$ is a backup vertex cover and $e$ is a supplier edge.}

  Let $e = (v_i,\star)$. If $i \leq k$, the guards on $v_i$ and $\star$ exchange positions. If $i > k$, we have the guard on the universal vertex move to $v_i$ via the supplier edge that was attacked. The guard on the backup vertex then moves to $\star$ along the bridge, leading to a original vertex cover. 

  \paragraph*{Case 5. $\mathcal{S}$ is a backup vertex cover and $e$ is a bridge edge.}

  The guards on $\dagger$ and $\star$ exchange places and the resulting configuration is again a backup vertex cover. 

  \paragraph*{Case 6. $\mathcal{S}$ is a original vertex cover and $e$ is a matching edge.}
  
  Let $e = (u_i,v_i)$. If $i \leq k$, the guards on $u_i$ and $v_i$ exchange positions. If $i > k$, and if $v_i$ has a guard, then the guards on $u_i$ and $v_i$ exchange positions. Otherwise let $j>k$ , $j\neq i$ be such that $v_j$ has a guard. Let $q \in [k]$ be such that $(x_q,x_i) \in E(G)$. We now perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $v_i$ along the matching edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; and 
    \item the guard on $u_j$ moves to $\star$ along a supplier edge.
  \end{itemize}

  Note that this new configuration of guards corresponds to a original vertex cover. 

  \paragraph*{Case 7. $\mathcal{S}$ is a original vertex cover and $e$ is a structural edge.}
  
   Let $e = (v_q,u_p)$. If $q \leq k$, then the guards on $v_q$ and $u_p$ exchange positions. If $q > k$, and if $v_q$ has a guard, then the guards on $u_p$ and $v_q$ exchange positions. Otherwise let $j\neq q$ be such that $v_j$ has a guard. Note that $j > k$. 
   
   If $p \leq k$, we perform the following sequence of moves:

  \begin{itemize}
    \item The guard on $u_p$ moves to $v_q$ along the structural edge that was attacked;
    \item the guard on $v_p$ moves to $u_p$ along a matching edge; 
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; and 
    \item the guard on $v_j$ moves to $\star$ along a supplier edge.
  \end{itemize}

  However, if $p > k$, then let $r \in [k]$ be such that $(x_r,x_p) \in E(G)$. We now perform the following sequence of moves:

  \begin{itemize}
    \item The guard on $u_p$ moves to $v_q$ along the structural edge that was attacked;
    \item the guard on $v_r$ moves to $u_p$ along a structural edge;
    \item the guard on the universal vertex moves to $v_r$ along a supplier edge; and 
    \item the guard on $v_j$ moves to $\star$ along a supplier edge.
  \end{itemize}

  Note that this new configuration of guards corresponds to a original vertex cover in all scenarios.

  \paragraph*{Case 8. $\mathcal{S}$ is a original vertex cover and $e$ is a sliding edge.}
  
   Let $i \in [n]$ and suppose $e = (u_i,w)$ for some $w \in C_i$. Suppose $i \leq k$. Let $j>k$ such that $v_j$ has a guard. Then we have the following sequence of moves. 

  \begin{itemize}
    \item the guard on $u_i$ moves to $w$ along the sliding edge that was attacked;
    \item the guard on $v_i$ moves to $u_i$ along a matching edge;
    \item the guard on the universal vertex moves to $v_i$ along a supplier edge; and 
    \item the guard on $u_j$ moves to $\star$ along a supplier edge.
  \end{itemize}
  
  Now suppose $i > k$ and suppose $v_i$ is such that $v_i$ has a guard. We now perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $w$ along the sliding edge that was attacked;
    \item the guard on $v_i$ moves to $u_i$ along a matching edge.
  \end{itemize}

  Now suppose $i > k$ and let $q \in [k]$ be such that $(x_q,x_i) \in E(G)$. Let $j>k$ and $j\neq i$ such that $v_j$ has a guard. We now perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $w$ along the sliding edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; and 
    \item the guard on $v_j$ moves to $\star$ along a supplier edge.
  \end{itemize}

  In both cases, the new configuration of the guards corresponds to a dependent vertex cover.
  
  \paragraph*{Case 9. $\mathcal{S}$ is a original vertex cover and $e$ is a supplier edge.}
  
  Let $e = (v_i,\star)$. If $i \leq k$, the guards on $v_i$ and $\star$ exchange positions. If $i > k$ and $v_i$ has a guard, the guard on $v_i$ and $\star$ exchange positions. If $i>k$ and $v_i$ does not have a guard, let $j>k$ and $j\neq i$ be such that $v_j$ has a guard. We have the guard on the universal vertex move to $v_i$ via the supplier edge that was attacked. The guard on $v_j$ then moves to $\star$ along a supplier edge, leading to another original vertex cover. 

  \paragraph*{Case 10. $\mathcal{S}$ is a original vertex cover and $e$ is a bridge edge.}

  Let $j>k$ be such that $v_j$ has a guard. The guard on $\star$ moves to $\dagger$ along the attacked bridge edge. The guard on $v_j$ moves to $\star$ along a supplier edge and the resulting configuration is a backup vertex cover. 

  \paragraph*{Case 11. $\mathcal{S}$ is a dependent vertex cover and $e$ is a matching edge.}
  
 Let $w\in C_j$ be such that $w$ has a guard. If $e=(u_j,v_j)$ is the edge which is attacked and $j > k$ then guard on $v_j$ moves to $u_j$ along the attacked edge $e$ and the guard on $w$ moves to $v_j$. Note that this new configuration corresponds to a original vertex cover.
 
 Let $e = (u_i,v_i)$ for some $i\neq j$. If $i \leq k$, the guards on $u_i$ and $v_i$ exchange positions and we have the same dependent vertex cover.
 
 If $i > k$, let $q \in [k]$ be such that $(x_q,x_i) \in E(G)$. We now perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $v_i$ along the matching edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge;
    \item the guard on $v_j$ moves to $\star$ along a supplier edge;
    \item the guard on $u_j$ moves to $v_j$ along a matching edge; and
    \item the guard on $w$ moves to $u_j$ along a sliding edge.
  \end{itemize}
 Note that this new configuration of guards corresponds to a original vertex cover. 

  \paragraph*{Case 12. $\mathcal{S}$ is a dependent vertex cover and $e$ is a structural edge.}
  
  Let $w\in C_j$ be such that $w$ has a guard.
  Suppose $e=(v_q,u_j)$. If $q<k$, guards on $v_q$ and $u_j$ exchange and we have the same dependent vertex cover. If $q>k$, guard on $u_j$ moves to $v_q$ along the attacked structural edge and guard on $w$ moves to $u_j$ along a sliding edge. Thus we have a original vertex cover.
  
   Let $e = (v_q,u_p)$ for some $p\neq j$. If $q \leq k$, then the guards on $v_q$ and $u_p$ exchange positions and we have the same dependent vertex cover. 
   If $q > k$ and $p\leq k$, then we perform the following sequence of moves:

  \begin{itemize}
    \item The guard on $u_p$ moves to $v_q$ along the structural edge that was attacked;
    \item the guard on $v_p$ moves to $u_p$ along a matching edge; 
    \item the guard on the universal vertex moves to $v_p$ along a supplier edge; 
    \item the guard on $u_j$ moves to $\star$ along a supplier edge;and
    \item the guard on $w$ moves to $u_j$ along a sliding edge.
  \end{itemize}

  However, if $p > k$, then let $r \in [k]$ be such that $(x_r,x_p) \in E(G)$. We now perform the following sequence of moves:

  \begin{itemize}
    \item The guard on $u_p$ moves to $v_q$ along the structural edge that was attacked;
    \item the guard on $v_r$ moves to $u_p$ along a structural edge;
    \item the guard on the universal vertex moves to $v_r$ along a supplier edge;
    \item the guard on $u_j$ moves to $\star$ along a supplier edge;and
    \item the guard on $w$ moves to $u_j$ along a sliding edge.
  \end{itemize}

  Note that this new configuration of guards corresponds to a original vertex cover.

  \paragraph*{Case 13. $\mathcal{S}$ is a dependent vertex cover and $e$ is a sliding edge.}
  
  Let $w\in C_j$ be such that $w$ has a guard.
  
  Suppose $e= (u_j,w)$ is the sliding edge which was attacked, then the guards exchange their positions and we have the same dependent vertex cover.
  Suppose $e= (u_j,z)$ for some $z\neq w$ is the sliding edge which was attacked, then the guard on $u_j$ moves to $z$ to defend the attack and the guard from $w$ moves to $u_j$, leading to a different dependent vertex cover. 
  
  Let $i \in [n]$ and suppose $e = (u_i,z)$ for some $z \in C_i$. Suppose $i \leq k$. Then we have the following sequence of moves. 

  \begin{itemize}
    \item the guard on $u_i$ moves to $z$ along the sliding edge that was attacked;
    \item the guard on $v_i$ moves to $u_i$ along a matching edge;
    \item the guard on the universal vertex moves to $v_i$ along a supplier edge;
    \item the guard on $v_j$ moves to $\star$ along a supplier edge; \item the guard on $u_j$ moves to $v_j$ along a matching edge; and
    \item the guard on $w$ moves to $u_j$.
  \end{itemize}

  Now suppose $i > k$ and let $q \in [k]$ be such that $(x_q,x_i) \in E(G)$. If $j \leq k$, we now perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $z$ along the sliding edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; 
    \item the guard on $v_j$ moves to $\star$ along a supplier edge;
    \item the guard on $u_j$ moves to $v_j$ along a matching edge; and
    \item the guard on $w$ moves to $u_j$.
  \end{itemize}
  
  On the other hand, suppose $i > k$ and $j > k$. We distinguish two scenarios here. If $x_i$ and $x_j$ are dominated by a common vertex in $G$, that is, there exists $q \in [k]$ be such that $(x_q,x_i) \in E(G)$ and $(x_q,x_j) \in E(G)$, then we perform the following sequence of moves:
  
  \begin{itemize}
    \item the guard on $u_i$ moves to $z$ along the sliding edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on $u_j$ moves to $v_q$ along another structural edge;
    \item the guard on $w$ moves to $u_j$.
  \end{itemize}

    Otherwise, suppose $x_i$ and $x_j$ are dominated by distinct vertices say $x_q$ and $x_p$ (respectively) in $G$, which is to say that there exists $p,q \in [k]$, $p \neq q$, such that $(x_q,x_i) \in E(G)$ and $(x_p,x_j) \in E(G)$. In this case, we perform the following sequence of moves:
    
  \begin{itemize}
    \item the guard on $u_i$ moves to $z$ along the sliding edge that was attacked;
    \item the guard on $v_q$ moves to $u_i$ along a structural edge;
    \item the guard on the universal vertex moves to $v_q$ along a supplier edge; 
    \item the guard on $v_p$ moves to $\star$ along a supplier edge;
    \item the guard on $u_j$ moves to $v_p$ along another structural edge;
    \item the guard on $w$ moves to $u_j$.
  \end{itemize}


  In all of the cases above, the new configuration of the guards corresponds to a dependent vertex cover.

  \paragraph*{Case 14. $\mathcal{S}$ is a dependent vertex cover and $e$ is a supplier edge.}
  
  Let $w\in C_j$ be such that $w$ has a guard. 
  
  If $e=(v_j,\star)$ and $j \leq k$, guards on $v_j$ and $\star$ exchange their positions and we again have the same dependent vertex cover. Suppose $j>k$, there exists $q\in[k]$ such that $(x_j,x_q) \in E(G)$. We now perform the following sequence of moves:
  \begin{itemize}
      \item The guard on $\star$ moves to $v_j$ along the attacked supplier edge;
      \item The guard on $v_q$ moves to $\star$ along a supplier edge;
      \item The guard on $u_j$ moves to $v_q$ along a structural edge; and 
      \item The guard on $w$ moves to $u_j$ along a sliding edge.
  \end{itemize} 
  Note that the resulting configuration is a original vertex cover.
   
  Let $e = (v_i,\star)$ where $i\neq j$. If $i \leq k$, the guards on $v_i$ and $\star$ exchange positions. 
  
  If $i>k$ and $j\leq k$, we have the following sequence of moves:
  \begin{itemize}
      \item The guard on the universal vertex moves to $v_i$ via the supplier edge that was attacked.
      \item The guard on $v_j$ moves to $\star$ along a supplier edge;
      \item The guard on $u_j$ moves to $v_j$ along a matching edge; and 
      \item The guard on $w$ moves to $u_j$ along a sliding edge.
  \end{itemize}
  
  Note that the resulting configuration is a original vertex cover.
  
  
  Suppose $i,j>k$, there exists $q\in[k]$ such that $(x_j,x_q)\in E(G)$. We now perform the following sequence of moves:
  \begin{itemize}
      \item The guard on $\star$ moves to $v_i$ along the attacked supplier edge;
      \item The guard on $v_q$ moves to $\star$ along a supplier edge;
      \item The guard on $u_j$ moves to $v_q$ along a structural edge; and 
      \item The guard on $w$ moves to $u_j$ along a sliding edge.
  \end{itemize} 
  
  Note that the resulting configuration is a original vertex cover.
  
  
  \paragraph*{Case 15. $\mathcal{S}$ is a dependent vertex cover and $e$ is a bridge edge.}
 Let $w\in C_j$ be such that $w$ has a guard. If $j\leq k$, we have the following sequence of moves:
 \begin{itemize}
     \item The guard on $\star$ moves to $\dagger$ along the attacked bridge edge;
     \item The guard on $v_j$ moves to $\star$ along a supplier edge;
     \item The guard on $u_j$ moves to $v_j$ along a matching edge;
     and
     \item The guard on $w$ moves to $u_j$ along a sliding edge.
 \end{itemize}
 
 Note that the resulting configuration is a backup vertex cover. 
 
 If $j>k$, there exists $q\in[k]$ such that $(x_j,x_q)\in E(G)$. We now perform the following sequence of moves:
 \begin{itemize}
     \item The guard on $\star$ moves to $\dagger$ along the attacked bridge edge;
     \item The guard on $v_q$ moves to $\star$ along a supplier edge;
     \item The guard on $u_j$ moves to $v_q$ along a structural edge;
     and
     \item The guard on $w$ moves to $u_j$ along a sliding edge.
 \end{itemize}
 
Note that the resulting configuration is a backup vertex cover. 
\end{proof}

% \nmtodo{See if we can compress ``it is possible to move every guard at most once to a neighboring vertex so that the attack on $e$ is defended''.}

\paragraph*{The Backward Direction.} Suppose $\langle H, \ell \rangle$ is a  \textsc{Yes}-instance of \EVC{}. We argue that $\langle G = (V,E),k \rangle$ is a \textsc{Yes}-instance of \DS.

We know that any sequence of edge attacks in $H$ can be defended by deploying at most $\ell = n + k + 2$ guards. Let $\mathcal{S}$ denote the initial placement of guards. 

We now consider two cases:

\paragraph*{Case 1. $\mathcal{S}$ contains the backup vertex.}

We already know that $\mathcal{S}$ contains all the partner vertices and the universal vertex by~\Cref{claim-invariant}. This accounts for the positions of $(n+1)$ guards. Additionally, because of the case we are in, we have one guard on the backup vertex. So the remaining $k$ guards occupy either original or dependent vertices. We propose that the corresponding vertices in $G$ form a dominating set. Specifically, let 

$$A^\prime := \{j ~|~ 1 \leq j \leq n \mbox{ and } v_i \in \mathcal{S}\}$$ 

and 

$$B^\prime := \{j ~|~ 1 \leq j \leq n \mbox{ and } C_j \cap \mathcal{S} \neq \emptyset\}.$$ 

We now claim that $S := \{x_i ~|~ i \in A^\prime \cup B^\prime\}$ is a dominating set in $G$. Suppose not. Then, let $x_t \in V(G)$ be a vertex that is not dominated by $S$. Let us attack the matching edge $(u_t,v_t)$. Note that $v_t$ is not occupied by a guard, and the guard on $u_t$ is forced to move to $v_t$ to defend this attack. However, observe that our assumption that $x_t$ is not dominated in $G$ implies that no neighbor of $u_t$ has a guard in $\mathcal{S}$. Therefore, this configuration now cannot be extended to a vertex cover, contradicting our assumption that every attack can be defended. Therefore, $S$ is indeed a dominating set in $G$, and it is straightforward to verify that $S$ has size at most $k$.

\paragraph*{Case 2. $\mathcal{S}$ does not contain the backup vertex.}

In this case, we attack the bridge. Let $\mathcal{S}^\prime$ denote the placement of the guards obtained by defending this attack. Note that $\mathcal{S}^\prime$ must contain the backup vertex. Now we argue as we did in the previous case. This concludes the proof in the reverse direction. 
\end{proof}
